Comparison of different sensor thicknesses and substrate materials for the monolithic small collection-electrode technology demonstrator CLICTD

Small collection-electrode monolithic CMOS sensors profit from a high signal-to-noise ratio and a small power consumption, but have a limited active sensor volume due to the fabrication process based on thin high-resistivity epitaxial layers. In this paper, the active sensor depth is investigated in the monolithic small collection-electrode technology demonstrator CLICTD. Charged particle beams are used to study the charge-collection properties and the performance of devices with different thicknesses both for perpendicular and inclined particle incidence. In CMOS sensors with a high-resistivity Czochralski substrate, the depth of the sensitive volume is found to increase by a factor two in comparison with standard epitaxial material and leads to significant improvements in the hit-detection efficiency and the spatial and time resolution.

==> charge.tex <==

\subsection{Signal}

\begin{figure*}[bpt]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\columnwidth]{Figures/charge/inPxl_charge_epi_202202.pdf}
		\caption{Epitaxial layer}
		\label{fig:clsChargeMap_epi}
	\end{subfigure}%
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\columnwidth]{Figures/charge/inPxl_charge_cz_202202.pdf}
		\caption{High-resistivity Czochralski}
		\label{fig:clsChargeMap_cz}
	\end{subfigure}%
	\caption{In-pixel representation of the seed pixel charge at the minimum detection threshold for a sensor with (a) epitaxial layer and (b) high-resistivity Czochralski substrate.
		Both sensors have a segmented n-implant and are biased at -6\,V/-6\,V at p-wells/substrate.}
	\label{fig:chargeMap}
\end{figure*}

The in-pixel representation of the cluster seed charge is presented in Fig.~\ref{fig:chargeMap} for a sensor with epitaxial layer and high-resistivity Czochralski substrate.
The seed pixel charge exhibits a maximum in the pixel centre and decreases towards the pixel corners due to increased charge sharing.
The larger signal of the sensor with high-resistivity Czochralski substrate is distinguishable in the entire pixel cell. 


